Causal Graph based Event Reasoning using Semantic Relation Experts

Understanding how events in a scenario causally connect with each other is important for effectively modeling and reasoning about events. But event reasoning remains a difficult challenge, and despite recent advances, Large Language Models (LLMs) still struggle to accurately identify causal connections between events. This struggle leads to poor performance on deeper reasoning tasks like event forecasting and timeline understanding. To address this challenge, we investigate the generation of causal event graphs (e.g., A enables B) as a parallel mechanism to help LLMs explicitly represent causality during inference. This paper evaluates both how to generate correct graphs as well as how graphs can assist reasoning. We propose a collaborative approach to causal graph generation where we use LLMs to simulate experts that focus on specific semantic relations. The experts engage in multiple rounds of discussions which are then consolidated by a final expert. Then, to demonstrate the utility of causal graphs, we use them on multiple downstream applications, and also introduce a new explainable event prediction task that requires a causal chain of events in the explanation. These explanations are more informative and coherent than baseline generations. Finally, our overall approach not finetuned on any downstream task, achieves competitive results with state-of-the-art models on both forecasting and next event prediction tasks.

==> sec4_exp.tex <==
\section{Experimental Setup}
\nb{How about we simply move the content under the methods section to a subsection under Evaluation?}

%generate explanations justifying the event likelihood predictions. 
%We believe that this step-by-step procedure would provide the model with a global understanding of the scenario in form of causal relations which would lead to better explanations.

%We compare our approach with different baseline settings and show that the structured explanations generated using graph structure are more informative, coherent and can be better capture the causal relations between events in the scenario. 

Our approach \method\ can be seen as a form of multi-step prompting that guides an LLM to identify causal connections that help it assess and explain the likelihood of the query event. We use a decoder-only instruction-following API-based model, GPT-4 \cite{openai2023gpt4}, as the base LLM for our experiments. We compare \method\ against different prompting approaches.

\subsection{Methods}\label{methods}
\nc{this is the only subsection, so either remove it or add a second subsection to address my comment above}

\nc{My big comment here: this is confusing \emph{models} from \emph{experiment setups}. The first CGEL is a model. The second "few shot causal chain" is also a model. But the third "few-shot causal chain with events" is a different experiment setting. It's given more input. Am I wrong? This needs to be cleaned up. What are the models and actual baselines ... and what are the different experiment settings? This needs to line up with the later Table 2 results.}

%We use decoder-only instruction-following API-based model, GPT-4 \cite{openai2023gpt4} as the base LLM for our experiments.
%We use different settings to generate event likelihood explanations and compare them on different criteria dimensions. 

\paragraph{Graph-based causal chain}
Our main contribution, \method\ captures explicit causal relations between events by creating its causal graph, and using it for likelihood prediction and later explanation. See Section \ref{sec:celp}.
%We are interested in generating structured event likelihood explanations that can capture explicit causal relations between events and serve as justifications as to why an event is likely. Our approach starts by first, extracting all events from a given news article, second, finding the casual relations between all events and generating a graph corresponding to those relations, third placing new events in the graph and finally, using paths in the graph to form explanations. 
All steps are executed using prompts provided to GPT-4.
The prompts we use for each step can be find in the Appendix \ref{prompts}.

Depending on where an event is placed, we can have multiple paths as explanations but we only choose one as the final event likelihood explanation. We can use different heuristics to pick a chain that contains the query event as the final explanation. We experimented with two: (a) select a random path and (b) select the longest path. 

\paragraph{One-shot causal chain}
In this baseline setting, we first provide GPT-4 with the in-context examples that include the text and causal chains (similar to the outputs of our graph-based approach) and then prompt it to directly generate causal chains containing the query event (prompts in Appendix \ref{prompts}). Similar to a graph-based causal chain approach, we would have multiple output chains, and use the same random path and longest path heuristics for picking the final explanation.

\paragraph{One-shot causal chain with events}
One of the main steps of our approach is extracting events that have already been described in the given news article. 
We therefore use another baseline setting, where GPT-4 is also given the list of events in the article and is then asked to generate the chains similar to the previous one-shot baseline. 
We use the same set of events that are extracted using GPT-4 for \method.

\paragraph{One-shot causal chain with reflection}
The reflection technique enables the model to analyze its own mistakes and improve its performance \cite{shinn2023reflexion}. In this setting we first generate causal chains and then ask the model to evaluate its previously generated chains for causality and check whether the events in the chain are causally related and if not, the model is asked to update its previously generated responses to better reflect the causal relations.


